TrajMatch: Towards Automatic Spatio-temporal Calibration for Roadside LiDARs through Trajectory Matching

Recently, it has become popular to deploy sensors such as LiDARs on the roadside to monitor the passing traffic and assist autonomous vehicle perception. Unlike autonomous vehicle systems, roadside sensors are usually affiliated with different subsystems and lack synchronization both in time and space. Calibration is a key technology which allows the central server to fuse the data generated by different location infrastructures, which can deliver improve the sensing range and detection robustness. Unfortunately, existing calibration algorithms often assume that the LiDARs are significantly overlapped or that the temporal calibration is already achieved. Since these assumptions do not always hold in the real world, the calibration results from the existing algorithms are often unsatisfactory and always need human involvement, which brings high labor costs. In this paper, we propose TrajMatch -- the first system that can automatically calibrate for roadside LiDARs in both time and space. The main idea is to automatically calibrate the sensors based on the result of the detection/tracking task instead of extracting special features. More deeply, we propose a mechanism for evaluating calibration parameters that is consistent with our algorithm, and we demonstrate the effectiveness of this scheme experimentally, which can also be used to guide parameter iterations for multiple calibration. Finally, to evaluate the performance of TrajMatch , we collect two dataset, one simulated dataset LiDARnet-sim 1.0 and a real-world dataset. Experiment results show that TrajMatch can achieve a spatial calibration error of less than 10cm and a temporal calibration error of less than 1.5ms.

==> reference.tex <==
%%%%%%%%%%%%%%%%%%%% other 
@article{arnold2020cooperative,
  title={Cooperative perception for 3D object detection in driving scenarios using infrastructure sensors},
  author={Arnold, Eduardo and Dianati, Mehrdad and de Temple, Robert and Fallah, Saber},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  year={2020},
  publisher={IEEE}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LiDAR calibration
@inproceedings{kim2021automated,
  title={Automated Extrinsic Calibration for 3D LiDARs with Range Offset Correction using an Arbitrary Planar Board},
  author={Kim, Junha and Kim, Changhyeon and Han, Youngsoo and Kim, H Jin},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={5082--5088},
  year={2021},
  organization={IEEE}
}

Your submission contained reference.bib and no associated reference.tex file.

@inproceedings{ppfnet,
  title={Ppfnet: Global context aware local features for robust 3d point matching},
  author={Deng, Haowen and Birdal, Tolga and Ilic, Slobodan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={195--205},
  year={2018}
}

@inproceedings{perfectMatch,
  title={The perfect match: 3d point cloud matching with smoothed densities},
  author={Gojcic, Zan and Zhou, Caifa and Wegner, Jan D and Wieser, Andreas},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5545--5554},
  year={2019}
}


@article{automated,
  title={Automated point cloud registration using visual and planar features for construction environments},
  author={Kim, Pileun and Chen, Jingdao and Cho, Yong K},
  journal={J. Comput. Civ. Eng},
  volume={32},
  number={2},
  pages={04017076},
  year={2018}
}




@Article{re_with_ground,
AUTHOR = {Yue, Rui and Xu, Hao and Wu, Jianqing and Sun, Renjuan and Yuan, Changwei},
TITLE = {Data Registration with Ground Points for Roadside LiDAR Sensors},
JOURNAL = {Remote Sensing},
VOLUME = {11},
YEAR = {2019},
NUMBER = {11},
ARTICLE-NUMBER = {1354},
URL = {https://www.mdpi.com/2072-4292/11/11/1354},
ISSN = {2072-4292},
ABSTRACT = {The Light Detection and Ranging (LiDAR) sensors are being considered as new traffic infrastructure sensors to detect road users&rsquo; trajectories for connected/autonomous vehicles and other traffic engineering applications. A LiDAR-enhanced traffic infrastructure system requires multiple LiDAR sensors around intersections, along with road segments, which can provide a seamless detection range at intersections or along arterials. Each LiDAR sensor generates cloud points of surrounding objects in a local coordinate system with the sensor at the origin, so it is necessary to integrate multiple roadside LiDAR sensors&rsquo; data into the same coordinate system. None of existing methods can integrate the data from roadside LiDAR sensors, because the extensive detection range of roadside sensors generates low-density cloud points and the alignment of roadside sensors is different from mapping scans or autonomous sensing systems. This paper presents a method to register datasets from multiple roadside LiDAR sensors. This approach innovatively integrates LiDAR datasets with 3D cloud points of road surface and 2D reference point features, so the method is abbreviated as RGP (Registration with Ground and Points). The RGP method applies optimization algorithms to identify the optimized linear coordinate transformation. This research considered the genetic algorithm (global optimization) and the hill climbing algorithm (local optimization). The performance of the RGP method and the different optimization algorithms was evaluated with field LiDAR sensors data. When the developed process can integrate data from roadside sensors, it can also register LiDAR sensors&rsquo; data on an autonomous vehicle or a robot.},
DOI = {10.3390/rs11111354}}


@article{curves_feature,
  title={Automated registration of dense terrestrial laser-scanning point clouds using curves},
  author={Yang, Bisheng and Zang, Yufu},
  journal={ISPRS journal of photogrammetry and remote sensing},
  volume={95},
  pages={109--121},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{intersectionFeature,
  title={Automated feature-based range registration of urban scenes of large scale},
  author={Stamos, Ioannis and Leordeanu, Marius},
  booktitle={2003 CVPR},
  volume={2},
  pages={II--Ii},
  year={2003},
  organization={IEEE}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% time have sync betweent sensors
@inproceedings{xie2018infrastructure,
  title={Infrastructure based calibration of a multi-camera and multi-lidar system using apriltags},
  author={Xie, Yuanfan and Shao, Rui and Guli, Popo and Li, Bo and Wang, Liang},
  booktitle={2018 IEEE Intelligent Vehicles Symposium (IV)},
  pages={605--610},

}



  
  
 @inproceedings{quenzel2016robust,
  title={Robust extrinsic calibration of multiple stationary laser range finders},
  author={Quenzel, Jan and Papenberg, Nils and Behnke, Sven},
  booktitle={2016 IEEE International Conference on Automation Science and Engineering (CASE)},
  pages={1332--1339},
  year={2016},
  organization={IEEE}
}
  

@inproceedings{pusztai2017accurate,
  title={Accurate calibration of LiDAR-camera systems using ordinary boxes},
  author={Pusztai, Zoltan and Hajder, Levente},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision Workshops},
  pages={394--402},
  year={2017}
} 
 
 @inproceedings{xue2019automatic,
  title={Automatic calibration of dual-LiDARs using two poles stickered with retro-reflective tape},
  author={Xue, Bohuan and Jiao, Jianhao and Zhu, Yilong and Zhen, Linwei and Han, Dong and Liu, Ming and Fan, Rui},
  booktitle={2019 IEEE International Conference on Imaging Systems and Techniques (IST)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}
 

 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% st 
 @article{pervsic2021spatiotemporal,
  title={Spatiotemporal multisensor calibration via gaussian processes moving target tracking},
  author={Per{\v{s}}i{\'c}, Juraj and Petrovi{\'c}, Luka and Markovi{\'c}, Ivan and Petrovi{\'c}, Ivan},
  journal={IEEE Transactions on Robotics},
  volume={37},
  number={5},
  pages={1401--1415},
  year={2021},
  publisher={IEEE}
}
 
 
 
@article{taylor2016motion,
  title={Motion-based calibration of multimodal sensor extrinsics and timing offset estimation},
  author={Taylor, Zachary and Nieto, Juan},
  journal={IEEE Transactions on Robotics},
  volume={32},
  number={5},
  pages={1215--1229},
  year={2016},
  publisher={IEEE}
}

@inproceedings{glas2015snapcat,
  title={SNAPCAT-3D: Calibrating networks of 3D range sensors for pedestrian tracking},
  author={Glas, Dylan F and Br{\v{s}}{\v{c}}i{\v{c}}, Dra{\v{z}}en and Miyashita, Takahiro and Hagita, Norihiro},
  booktitle={2015 IEEE international conference on robotics and automation (ICRA)},
  pages={712--719},
  year={2015},
  organization={IEEE}
}

@INPROCEEDINGS{6385620,
  author={Schenk, Konrad and Kolarow, Alexander and Eisenbach, Markus and Debes, Klaus and Gross, Horst-Michael},
  booktitle={2012 IEEE/RSJ International Conference on Intelligent Robots and Systems}, 
  title={Automatic calibration of a stationary network of laser range finders by matching movement trajectories}, 
  year={2012},
  volume={},
  number={},
  pages={431-437},
  doi={10.1109/IROS.2012.6385620}}
  
  
  @inproceedings{vi-eye,
  title={VI-eye: semantic-based 3D point cloud registration for infrastructure-assisted autonomous driving},
  author={He, Yuze and Ma, Li and Jiang, Zhehao and Tang, Yi and Xing, Guoliang},
  booktitle={Proceedings of the 27th Annual International Conference on Mobile Computing and Networking},
  pages={573--586},
  year={2021}
}

@ARTICLE { Radar-Camera ,
  author={Du, Yuchuan and Qin, Bohao and Zhao, Cong and Zhu, Yifan and Cao, Jing and Ji, Yuxiong},
  journal={IEEE Transactions on Intelligent Transportation Systems}, 
  title={A Novel Spatio-Temporal Synchronization Method of Roadside Asynchronous MMW Radar-Camera for Sensor Fusion}, 
  year={2021},
  volume={},
  number={},
  pages={1-12},
  doi={10.1109/TITS.2021.3119079}}
  
  
  

@article{WU2091105,
title = {Quantifying what goes unseen in instrumented and autonomous vehicle perception sensor data – A case study},
journal = {Transportation Research Part C: Emerging Technologies},
volume = {107},
pages = {105-119},
year = {2019},
issn = {0968-090X},
author = {Mo Wu and Benjamin Coifman},
}  

@article{rehder2016general,
  title={A general approach to spatiotemporal calibration in multisensor systems},
  author={Rehder, Joern and Siegwart, Roland and Furgale, Paul},
  journal={IEEE Transactions on Robotics},
  volume={32},
  number={2},
  pages={383--398},
  year={2016},
  publisher={IEEE}
}


@article{li2014online,
  title={Online temporal calibration for camera--IMU systems: Theory and algorithms},
  author={Li, Mingyang and Mourikis, Anastasios I},
  journal={The International Journal of Robotics Research},
  volume={33},
  number={7},
  pages={947--964},
  year={2014},
  publisher={SAGE Publications Sage UK: London, England}
}


@article{lidartag,
  title={LiDARTag: A real-time fiducial tag system for point clouds},
  author={Huang, Jiunn-Kai and Wang},
  volume={6},
  number={3},
  pages={4875--4882},
  year={2021},
}


@inproceedings{qin2018online,
  title={Online temporal calibration for monocular visual-inertial systems},
  author={Qin, Tong and Shen, Shaojie},
  booktitle={2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={3662--3669},
  year={2018},
  organization={IEEE}
}

@inproceedings{kelly2014general,
  title={A general framework for temporal calibration of multiple proprioceptive and exteroceptive sensors},
  author={Kelly, Jonathan and Sukhatme, Gaurav S},
  booktitle={Experimental Robotics},
  pages={195--209},
  year={2014},
  organization={Springer}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 数据集
@misc{nuscenes,
  author = {} ,
  title = { Leaderboard of detection on nuScenes  },
  howpublished = "\url{https://www.nuscenes.org/object-detection?externalData=all&mapData=all&modalities=Any}",
  year = {[n.d.]}
}



@misc{RS-LiDARLIte,
  author = {} ,
  title = { RS-LiDAR\_LIte },
  howpublished = "\url{https://www.robosense.ai/rslidar/RS-Ruby_Lite}",
  year = {[n.d.]}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% detection 
@inproceedings{pointnet,
  title={Pointnet: Deep learning on point sets for 3d classification and segmentation},
  author={Qi, Charles R and Su },
  booktitle={CVPR},
  pages={652--660},
  year={2017}
}

@inproceedings{deng2021voxel,
  title={Voxel r-cnn: Towards high performance voxel-based 3d object detection},
  author={Deng, Jiajun},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={2},
  pages={1201--1209},
  year={2021}
}


@inproceedings{pointpillars,
  title={Pointpillars: Fast encoders for object detection from point clouds},
  author={Lang, Alex H and Vora, Sourabh and Caesar, Holger and Zhou, Lubing and Yang, Jiong and Beijbom, Oscar},
  booktitle={CVPR},
  pages={12697--12705},
  year={2019}
}



@ARTICLE{9839508,
  author={Li, Yao and Deng, Jiajun and Zhang, Yu and Ji, Jianmin and Li, Houqiang and Zhang, Yanyong},
  journal={IEEE Robotics and Automation Letters}, 
  title={${\mathsf{EZFusion}}$: A Close Look at the Integration of LiDAR, Millimeter-Wave Radar, and Camera for Accurate 3D Object Detection and Tracking}, 
  year={2022},
  volume={7},
  number={4},
  pages={11182-11189},
  doi={10.1109/LRA.2022.3193465}} 
  
  
@inproceedings{AB3DMOT,
    author = {Weng, Xinshuo and Wang, Jianren and Held, David and Kitani, Kris},
    year = {2020},
    month = {08},
    pages = {},
    title = {AB3DMOT: A Baseline for 3D Multi-Object Tracking and New Evaluation Metrics}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% trajectories minning 


@Article{survey_trajector_cluster,
    author={Yuan, Guan and Sun, Penghui and Zhao, Jie and Li, Daxing and Wang, Canwei},
    title={A review of moving object trajectory clustering algorithms},
    journal={Artificial Intelligence Review},
    year={2017},
    month={Jan},
    day={01},
    volume={47},
    number={1},
    pages={123-144},
    issn={1573-7462},
}





@article{TrajSimilarity,
author = {Sousa, Roniel S. De and Boukerche, Azzedine and Loureiro, Antonio A. F.},
title = {Vehicle Trajectory Similarity: Models, Methods, and Applications},
year = {2020},
issue_date = {September 2021},
publisher = {Association for Computing Machinery},
volume = {53},
number = {5},
issn = {0360-0300},
journal = {ACM Comput. Surv.},
}



@inproceedings{kong2015kinematic,
  title={Kinematic and dynamic vehicle models for autonomous driving control design},
  author={Kong, Jason and Pfeiffer, Mark and Schildbach, Georg and Borrelli, Francesco},
  booktitle={2015 IEEE intelligent vehicles symposium (IV)},
  pages={1094--1099},
  year={2015},
  organization={IEEE}
}


@ARTICLE{ICP,
  author={Besl, P.J. and McKay, Neil D.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={A method for registration of 3-D shapes}, 
  year={1992},
  volume={14},
  number={2},
  pages={239-256},
  doi={10.1109/34.121791}}
  
  
  
@inproceedings{ndt,
  title={The normal distributions transform: A new approach to laser scan matching},
  author={Biber, Peter and Stra{\ss}er, Wolfgang},
  booktitle={Proceedings 2003 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS 2003)(Cat. No. 03CH37453)},
  volume={3},
  pages={2743--2748},
  year={2003},
  organization={IEEE}
} 
 
 
@incollection{4pcs,
  title={4-points congruent sets for robust pairwise surface registration},
  author={Aiger, Dror and Mitra, Niloy J and Cohen-Or, Daniel},
  booktitle={ACM SIGGRAPH 2008 papers},
  pages={1--10},
  year={2008}
}

@article{k4pcs,
  title={Keypoint-based 4-points congruent sets--automated marker-less registration of laser scans},
  author={Theiler, Pascal Willy and Wegner, Jan Dirk and Schindler, Konrad},
  journal={ISPRS journal of photogrammetry and remote sensing},
  volume={96},
  pages={149--163},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{SAC-IA,
  title={Fast point feature histograms (FPFH) for 3D registration},
  author={Rusu, Radu Bogdan and Blodow, Nico and Beetz, Michael},
  booktitle={2009 IEEE international conference on robotics and automation},
  pages={3212--3217},
  year={2009},
  organization={IEEE}
}


@inproceedings{pcl,
  title={3d is here: Point cloud library (pcl)},
  author={Rusu, Radu Bogdan and Cousins, Steve},
  booktitle={2011 IEEE international conference on robotics and automation},
  pages={1--4},
  year={2011},
  organization={IEEE}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 模拟器

@inproceedings{CARLA,
  title={CARLA: An open urban driving simulator},
  author={Dosovitskiy, Alexey and Ros, German and Codevilla, Felipe and Lopez, Antonio and Koltun, Vladlen},
  booktitle={Conference on robot learning},
  pages={1--16},
  year={2017},
  organization={PMLR}
}


@article{sumo,
  title={Recent development and applications of SUMO-Simulation of Urban MObility},
  author={Krajzewicz, Daniel and Erdmann, Jakob and Behrisch, Michael and Bieker, Laura},
  journal={International journal on advances in systems and measurements},
  volume={5},
  number={3\&4},
  year={2012},
  publisher={Citeseer}
}




@article{ZAI201715,
title = {Pairwise registration of TLS point clouds using covariance descriptors and a non-cooperative game},
journal = {ISPRS Journal of Photogrammetry and Remote Sensing},
volume = {134},
pages = {15-29},
year = {2017},
issn = {0924-2716},
author = {Dawei Zai and Jonathan Li},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 评估指标
@inproceedings{RRE_RTE,
  title={Are we ready for autonomous driving? the kitti vision benchmark suite},
  author={Geiger, Andreas and Lenz, Philip and Urtasun, Raquel},
  booktitle={2012 IEEE conference on computer vision and pattern recognition},
  pages={3354--3361},
  year={2012},
  organization={IEEE}
}




@inproceedings{deep_global_regi,
  title={Deep global registration},
  author={Choy, Christopher and Dong, Wei and Koltun, Vladlen},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2514--2523},
  year={2020}
}



@inproceedings{elbaz20173d,
  title={3D point cloud registration for localization using a deep neural network auto-encoder},
  author={Elbaz, Gil and Avraham, Tamar and Fischer, Anath},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4631--4640},
  year={2017}
}



@article{liu2018progress,
  title={Progress and consideration of high precision road navigation map},
  author={Liu, Jingnan and Wu, Hangbin and Guo, Chi and Zhang, Hongmin and Zuo, Wenwei and Yang, Cheng},
  journal={Strategic Study of Chinese Academy of Engineering},
  volume={20},
  number={2},
  pages={99--105},
  year={2018}
}
